A Lightweight Framework for Adaptive Retrieval In Code Completion With Critique Model

Recent advancements in Retrieval-Augmented Generation have significantly enhanced code completion at the repository level. Various RAG-based code completion systems are proposed based on different design choices. For instance, gaining more effectiveness at the cost of repeating the retrieval-generation process multiple times. However, the indiscriminate use of retrieval in current methods reveals issues in both efficiency and effectiveness, as a considerable portion of retrievals are unnecessary and may introduce unhelpful or even harmful suggestions to code language models. To address these challenges, we introduce CARD, a lightweight critique method designed to provide insights into the necessity of retrievals and select the optimal answer from multiple predictions. CARD can seamlessly integrate into any RAG-based code completion system. Our evaluation shows that CARD saves 21% to 46% times of retrieval for Line completion, 14% to 40% times of retrieval for API completion, and 6% to 46.5% times of retrieval for function completion respectively, while improving the accuracy. CARD reduces latency ranging from 16% to 83%. CARD is generalizable to different LMs, retrievers, and programming languages. It is lightweight with training in few seconds and inference in few milliseconds.

==> sections/pre-bak.tex <==

\section{Preliminaries}
\paragraph{Iterative RAG}
%In this setting, RAG for coding can be formulated as XXX. Our adaptive RAG can be formulated as XXX. The core part is to design a function/train a model to optimize XXX.
% \subsubsection{Iterative RAG}
Considering the scenario where the LM $\mathcal{M}_\theta$ (parameterized by $\theta$) is interacted with prompt $X\in\mathcal{X}$ and generate the response $\hat{y}=(\hat{y}_1,\hat{y}_2,\cdots,\hat{y}_N)\in\mathcal{Y}$, where $N$ is the total number of generated tokens. The zero-shot generation can be formulated as $\hat{y}=\mathcal{M_\theta}(X)$.

% \subsubsection{Repository-level Code Completion} 
In the above setting, the repository-level code completion task can be denoted as $(X, y, F)$, where $X$ is the in-file context (code to be completed), $y$ is the ground truth response of prompt $X$, and $F$ denotes the set of other files in the repository. 

One-time RAG for coding can be regarded as RG-1 formulation in \citet{zhang2023repocoder}, including \textit{indexing}, \textit{query formation}, \textit{retrieval} and \textit{generation}. The retrieved code segments $C$ from $F$ would be added to the $X$, thus the task is formulated as $y=\mathcal{M}_\theta(C, X), C=\mathcal{R}(\mathcal{Q}(X), F)$, where $\mathcal{R}$ and $\mathcal{Q}$ denotes the process of \textit{retrieval} and \textit{query formation} respectively. Iterative RAG utilizes the generated code completion to form the query, thus $C^{i+1}$ (query in the $i+1$-th iteration) would be conditioned on $y^i$ ($y$ generated in the $i$-th iteration). Formally, the generation at the $i$-th iteration can be formulated as $\hat{y}^i=\mathcal{M}_\theta(C^{i},X)$, $C^{i}=\mathcal{R}(\mathcal{Q}(X, \hat{y}^{i-1}), F)$.



\subsection{Preliminaries}
\paragraph{Uncertainty estimation for LMs}
When $\mathcal{M}_\theta$ is used for downstream tasks, such as question answering and code completion, the uncertainty estimation usually comes with a scoring function evaluating the quality of the generated response:
\begin{equation}\label{equ:score_func}
S(\cdot,\cdot):\mathcal{Y}\times\mathcal{Y}\rightarrow[0,1]  \nonumber
\end{equation}
For each observed pair $(X,y)$, the scoring function evaluates the response with the score $s=S(y,\hat{y})$. The task of \textit{uncertainty estimation} for LMs is defined in~\cite{liu2024uncertainty} as the learning/fitting a function $g$ where
$$g(X,y)\approx \mathbb{E}[S(y,\hat{y})|X,y]$$Note that $g(\cdot,\cdot)$ is independent of the ground truth $y$, thus broadening the applicability and practicality of the uncertainty estimator.

